The Move Borrow Checker

The Move language provides abstractions for programming with digital assets via a mix of value semantics and reference semantics. Ensuring memory safety in programs with references that access a shared, mutable global ledger is difficult, yet essential for the use-cases targeted by Move. The language meets this challenge with a novel memory model and a modular, intraprocedural static reference safety analysis that leverages key properties of the memory. The analysis ensures the absence of memory safety violations in all Move programs (including ones that link against untrusted code) by running as part of a load-time bytecode verification pass similar to the JVM [12] and CLR [15]. We formalize the static analysis and prove that it enjoys three desirable properties: absence of dangling references, referential transparency for immutable references, and absence of memory leaks.

==> fig-rules-global.tex <==
\newcommand{\mycomment}[1]{}

\begin{figure*}
\begin{centerframe}
\begin{small}

\pcrule[]
  {
    \typeof{a}{\addresstype}\sep
    \typeof{v}{t}\sep
    \tup{t,a} \notin \dom{G}\sep
    c\notin\dom{M}
  }
  {\ao{\movetoCmd}{t}}
  {\st{L,\stackht{\stackht{a}{v}}{S},M,G}}
  {\st{L,S,\mset{M}{c}{v},\gset{G}{\tup{t,a}}{c}}}\hspace{5mm}
\pcrule[]
  {
    \typeof{a}{\addresstype}\sep
    \tup{t,a} \in \dom{G}
  }
  {\ao{\movetoCmd}{t}}
  {\st{L,\stackht{\stackht{a}{v}}{S},M,G}}
  {\execerror{}}
  \bigskip

\pcrule[]
  {
    \typeof{a}{\addresstype}\sep
    \gread{G}{\tup{t,a}} = c\sep
    \mread{M}{c}=v
  }
  {\ao{\movefromCmd}{t}}
  {\st{L,\stackht{a}{S},M,G}}
  {\st{L,\stackht{v}{S},\mdel{M}{c},\gdel{G}{\tup{t,a}}}}\hspace{5mm}
\pcrule[]
  {
    \typeof{a}{\addresstype}\sep
    \tup{t,a} \notin \dom{G}
  }
  {\ao{\movefromCmd}{t}}
  {\st{L,\stackht{a}{S},M,G}}
  {\execerror{}}
  \bigskip

\pcrule[]
  {
    \typeof{a}{\addresstype}\sep
    \gread{G}{\tup{t,a}} = c
  }
  {\ao{\borrowglobalCmd}{t}}
  {\st{L,\stackht{a}{S},M,G}}
  {\st{L,\stackht{\rft{c}{[]}}{S},M,G}}\hspace{5mm}
\pcrule[]
  {
    \typeof{a}{\addresstype}\sep
    \tup{t,a} \notin \dom{G}
  }
  {\ao{\borrowglobalCmd}{t}}
  {\st{L,\stackht{a}{S},M,G}}
  {\execerror{}}
  \bigskip

\pcrule[]
  {
    b = \tup{t,a} \in \dom{G}
  }
  {\ao{\existsCmd}{t}}
  {\st{L,\stackht{a}{S},M,G}}
  {\st{L,\stackht{b}{S},M,G}}
\caption{\label{fig:opsemAcc}Operational Semantics of \move: Global state operations}
\end{small}
\end{centerframe}
\end{figure*}


==> fig-rules-pc.tex <==
\begin{figure*}
\begin{centerframe}
\pcrule[]
  {
    \pcstep{\progloc{\proc}{\pc}}{\st{M,L,S}}{\st{M',L',S'}}
  }
	{\program}{\st{M,\stackht{(\proc, \pc, L)}{F},S}}{\st{M',\stackht{(\proc, \pc + 1, L')}{F},S'}}
  \bigskip

\pcrule[]
  {
	  \progloc{\proc}{\pc}=\ao{\jumpCmd}{\pc'}
  }
	{\program}{\st{M,\stackht{(\proc, \pc, L)}{F},S}}{\st{M,\stackht{(\proc, \pc', L)}{F},S}}\hspace{5mm}
\pcrule[]
  {
	  \progloc{\proc}{\pc}=\ao{\branchCmd}{\pc_1, \pc_2},
    \pc' = \ite{\mread{M}{c}=\true}{\pc_1}{\pc_2}
  }
	{\program}{\st{M,\stackht{(\proc, \pc, L)}{F},\stackht{c}{S}}}{\st{M,\stackht{(\proc, \pc', L)}{F},S}}
  \bigskip

\pcrule[]
  {
    x = (\proc, \pc, L)\sep
    \progloc{\proc}{\pc}=\ao{\callCmd}{\proc'}
  }
  {\program}{\st{M,\stackht{x}{F},\stackht{\overline{v}}{S}}}{\st{M,\stackht{(\proc', 0, \reverse{\overline{v}})}{\stackht{x}{F}},S}}\hspace{5mm}
\pcrule[]
  {
    x = (\proc, \pc, L)\sep
	  \progloc{\proc}{\pc}=\returnCmd
  }
	{\program}{\st{M,\stackht{x}{\stackht{(\proc', \pc', L')}{F}},S}}{\st{M,\stackht{(\proc', \pc'+1, L')}{F},S}}
\caption{\label{fig:pcrules} Control-flow rules}
\end{centerframe}
\end{figure*}


==> proof.tex <==
\newcommand{\halfstep}{\rightharpoonup}
\newcommand{\Base}{\mathit{Base}}
\newcommand{\hole}{\square}

We prove soundness of the borrow checker (Theorem \ref{type-sound-thm})
by showing that
the inductive invariant between concrete and abstract states
is preserved by execution of any well-typed program.
This short addendum to the submitted paper
describes the proof and gives the key elements
of the technical argument.

The proof of Theorem \ref{type-sound-thm} is decomposed into smaller lemmas.
Recall that a concrete state contains the procedure call stack, procedure name,
and a program counter that identifies the next instruction.
The first lemma shows that if we execute any instruction next
from any concrete state, the invariant is preserved between the
new concrete state and an abstract state based on the
borrow checker rules.
This state must be in the $\below$ relation with
with the next program annotation.
We next use another lemma relating $\below$ and
the invariant to prove the theorem.

We beging with a simpler helper lemma that states an important
and useful fact connecting borrow graphs and reference types.
\begin{manuallemma}{0}
  \label{no-path-imm-to-mut}
  Suppose $\absState = \abs{\concState} = \st{\hat{L},\hat{S},B}$ and
  $\inv(\concState,\absState)$.
  If $m,n \in \dom{\absState}$ are distinct, $\absState(n) \in \mutreftype$,
  and there is a path in $B$ realizable in $\concState$ from $m$ to $n$,
  then $\absState(m) \not \in \immreftype$.
\end{manuallemma}
\jm{I think this should be $\absState = \abs{\concState} = \st{\hat{P},\hat{S},B}$
in the statement of the lemma, with $\hat{P}$ instead of $\hat{L}$, for 
consistency.}

\begin{proof}[Proof of Lemma \ref{no-path-imm-to-mut}]
If there is a path in $B$ realizable in $\concState$ from $m$ to $n$,
then $\concState(m) \leq \concState(n)$.
We know that $\absState(n) \not \in \immreftype$.
We also know that since the borrow graph in $\absState$ is acyclic,
there is no path in it from $n$ to $m$.
The definition of referential transparency part of $\inv$ allows us to conclude
that $\absState(m) \not \in \immreftype$.
\end{proof}

We now introduce helpful notation.
Recall that all bytecode instructions other than call and return
operate on a local state $\st{L,S,M}$, where
$L$ is a local store from the top frame of a concrete state $\st{\stackht{(\proc, \pc, L)}{P},S,M}$.
A local instruction changes local states $\st{L,S,M} \rightarrow \st{L',S',M'}$
resulting in a state change
\[
\st{\stackht{(\proc, \pc, L)}{P},{S},M} \rightarrow
   \st{\stackht{(\proc, \pc+1, L')}{P},{S'},M'}
 \]
when extended to full states.

In our static analysis, a local instruction defines an associated transition
$\st{\hat{L}_1,\hat{S}_1,B_1} \rightarrow \st{\hat{L}_2,\hat{S}_2,B_2}$
of abstract local states,expressed by the borrow checker rules.
To extend a local abstract state transition to full states,
we view that transition as occurring on the top of any additional abstract call stack.
However, unlike the concrete semantics, the abstract semantics are formulated using
only a top fragment of the operand stack and a local borrow graph that must be integrated
into the full  abstract state.

Suppose $\concState = \st{\stackht{(\proc, \pc, L)}{P},\_,\_}$ has a nonempty call stack.
We define
$\Base(\concState) = \st{\stackht{(\proc, \pc, \hole)}{\absframe{P}},\absstack{P},\absgraph{P}{\len{P}+1}}$.
$\Base(\concState)$ is an \emph{abstract state with a hole}.
It is useful to view the abstract state $\absState = \abs{\concState}$ in the form
\[
\absState = \Base(\concState) \dagger \st{\hat{L},\hat{S},B}
\]
where $\lstates{\proc}[\pc] = \st{\hat{L},\hat{S},B}$.
The operation $\dagger$ in $\Base(\concState) \dagger \st{\hat{L},\hat{S},B}$ fills the hole $\hole$ with
$\hat{L}$, appends $\hat{S}$ to the operand stack of $\Base(\concState)$, and adds the borrow edges
in $\rename{B}{R}$ to the borrow graph of $\Base(\concState)$,
where
$R = \{(\psloc(0,y),\psloc(\len{P},y)) \mid y \in \dom{\hat{L}}\}\ \cup
\{(\osloc(x),\osloc(x + \len{\absstack{P}})) \mid x \in 0..\len{\hat{S}}\}$.
We will often find it useful in our proof to construct the abstract state
$ \Base(\concState) \dagger \ls'$ where $\ls'$ is different from $\lstates{\proc}[\pc]$.
The following lemma indicates a key property of $\Base$ and
$\dagger$.
\begin{manuallemma}{1}
\label{type-weakening-lemma}
If
\begin{itemize}
\item
$\inv(\concState', \Base(\concState')\dagger \st{\hat{L}_1,\hat{S}_1,B_1})$
\item
$\st{\hat{L}_1,\hat{S}_1,B_1} \below \st{\hat{L}_2,\hat{S}_2,B_2}$
\end{itemize}
then
$\inv(\concState', \Base(\concState')\dagger \st{\hat{L}_2,\hat{S}_2,B_2})$.
\end{manuallemma}

\begin{proof}[Proof of Lemma \ref{type-weakening-lemma}]
Let $\absState_1 = \Base(\concState')\dagger \st{\hat{L}_1,\hat{S}_1,B_1})$
and $\absState_2 = \Base(\concState')\dagger \st{\hat{L}_2,\hat{S}_2,B_2})$.
The definition of $\below$ indicates that if
$\st{\hat{L}_1,\hat{S}_1,B_1} \below \st{\hat{L}_2,\hat{S}_2,B_2}$
then $\hat{L}_1 = \hat{L}_2$, $\hat{S}_1 = \hat{S}_2$,
and each edge in $B_1$ is subsumed by some edge in $B_2$.
Thus, the call stacks and operand stacks of $\absState_1$ and $\absState_2$ are identical
and each edge in the global borrow graph of $\absState_1$ is subsumed by some edge in
the global  borrow graph of $\absState_2$.
The preservation of $\inv$ follows from the definition of subsumption of
a borrow edge.
\end{proof}

To aid our proof, we define an auxiliary transition relation
$\program \vdash \concState \halfstep \concState$.
We view a transition $\program \vdash \concState \rightarrow \concState'$
as happening in two steps.
In the first step, the instruction pointed to by the program counter at
the top of the call stack in $\concState$ is executed to change parts
of the state to yield $\concState^-$
without adjusting the program counter to point to the next instruction.
In the second step, the program counter in $\concState^-$
is adjusted to yield $\concState'$ and move to the next instruction.
We write $\program \vdash \concState \halfstep \concState^-$
to denote the first part of this two-step process.
The concrete states $\concState^-$ and $\concState'$
coincide in the two cases when
the call stack in $\concState'$ is empty or
$\concState'$ is obtained from $\concState$ by executing a
call instruction;
in these two cases,
$\program \vdash \concState \rightarrow \concState'$
is a single step.

The following two lemmas together state that the transformation
of the abstract state when a local instruction is executed preserves $\inv$.
The proof of Lemma~\ref{type-sound-lemma-local}
is provided later in this document.
\begin{manuallemma}{2}
\label{type-sound-lemma-local}
If
\begin{itemize}
\item
$\concState = \st{\stackht{(\proc, \pc, \_)}{\_},\_,\_}$
\item
$\inv(\concState,\abs{\concState})$
\item
$\program \vdash \concState \halfstep \concState'$ by a local instruction
\item
$\proc,\bcodes{\proc}[\pc] \vdash \lstates{\proc}[\pc] \rightarrow
\st{\hat{L},\hat{S},B}$
\end{itemize}
then
$\inv(\concState',\Base(\concState) \dagger \st{\hat{L},\hat{S},B})$.
\end{manuallemma}

\begin{manuallemma}{3}
\label{type-sound-lemma}
If
\begin{itemize}
\item
$\inv(\concState,\abs{\concState})$
\item
$\program \vdash \concState \halfstep \concState'$
\item
$\program \vdash \concState \rightarrow (\stackht{\st{\proc,\pc,\_}}{\_},\_,\_)$
\end{itemize}
then there exists $\st{\hat{L},\hat{S},B}$
such that
\begin{itemize}
\item
$\inv(s',\Base(s') \dagger \st{\hat{L},\hat{S},B})$
\item
$\st{\hat{L},\hat{S},B} \below \lstates{\proc}[\pc]$.
\end{itemize}
\end{manuallemma}

\begin{proof}[Proof of Lemma \ref{type-sound-lemma}]
If $\program \vdash \concState \halfstep \concState'$ by a local instruction,
then $\Base(\concState) = \Base(\concState')$ and
we get the result from Lemma~\ref{type-sound-lemma-local}
and the definition of $\program$ being well-typed.
The case for $\branchCmd$ is similar.

Suppose $\program \vdash \concState \halfstep \concState'$ via
$\ao{\callCmd}{\proc'}$.
We argue
$\inv(\concState',\Base(\concState') \dagger \lstates{\proc'}[0])$ holds.
The proof follows since $\below$ is reflexive.

Suppose $\program \vdash \concState \halfstep \concState'$ via
$\returnCmd$ and $\bcodes{\proc}[\pc] = \ao{\callCmd}{\proc'}$.
Suppose
$\abs{\concState'} = \Base(\concState') \dagger \st{\hat{L}_1,\hat{S}_1,B_1}$.
Then, we know that
$\bcodes{\proc}[\pc - 1] = \ao{\callCmd}{\proc'}$,
$\lstates{\proc}[\pc - 1] = \st{\hat{L}_1,\hat{S}_1,B_1}$, and
there exists $\st{\hat{L}_2,\hat{S}_2,B_2}$ such that
$\proc, \ao{\callCmd}{\proc'} \vdash \st{\hat{L}_1,\hat{S}_1,B_1} \rightarrow \st{\hat{L}_2,\hat{S}_2,B_2}$.
We argue that $\inv(\concState',\Base(\concState') \dagger \st{\hat{L}_2,\hat{S}_2,B_2})$
holds using the typing argument
for $\returnCmd$ in $\proc'$ and $\ao{\callCmd}{\proc'}$ in $\proc$.
Since $\program$ is well-typed, we also know that $\st{\hat{L}_2,\hat{S}_2,B_2} \subseteq \lstates{\proc}[\pc]$
and the proof follows.
\end{proof}

Lemmas~\ref{type-sound-lemma-local} and~\ref{type-sound-lemma}
are combined to prove the Theorem~\ref{type-sound-thm}.
\begin{manualtheorem}{1}
\label{type-sound-thm}
Let program $\program$ be well-typed.
If $\concState$ is a concrete state with $\inv(\concState,\abs{\concState})$
and $\program \vdash \concState \rightarrow \concState'$,
then $\inv(\concState',\abs{\concState'})$.
\end{manualtheorem}

\begin{proof}[Proof of Theorem \ref{type-sound-thm}]
Let program $\program$ be well-typed.
Let $\concState$ be a concrete state with $\inv(\concState,\abs{\concState})$
and $\program \vdash \concState \rightarrow \concState'$.
If the transition is due to \rulename{Emp}, the call stack
and operand stack in $\concState'$ are both empty.
Therefore, $\abs{\concState'} = \st{[],[],\{\}}$ and
$\inv(\concState',\abs{\concState'})$ holds trivially.

In all cases other than \rulename{Emp}, the call stack in $\concState'$
is nonempty.
Let $\concState \halfstep \concState^-$ and let the top frame of
the call stack of $\concState'$ be $\st{\proc,\pc,\_}$.
We use Lemma~\ref{type-sound-lemma} to find
$\st{\hat{L},\hat{S},B} \below \lstates{\proc}[\pc]$
such that $\inv(\concState^-,\Base(\concState^-) \dagger \st{\hat{L},\hat{S},B})$.
We use Lemma~\ref{type-weakening-lemma} to conclude that
$\inv(\concState^-,\Base(\concState^-) \dagger \lstates{\proc}[\pc])$.
By replacing the program counter in the top frame of the call stack of
$\concState^-$, we get $\concState'$.
By replacing the program counter in the top frame of the call stack of
$\Base(\concState^-) \dagger \lstates{\proc}[\pc])$,
we get $\abs{\concState'}$.
Therefore, we get $\inv(\concState', \abs{\concState'})$.
\end{proof}

\begin{proof}[Proof of Lemma \ref{type-sound-lemma-local}]
Let
$\absState  = \abs{\concState}  = \st{\stackht{(\proc, \pc, \hat{L})}{\hat{P}},\hat{S},B}$.
Note that $\absState$ has the same procedure name and program counter
in the top of the call stack as $\concState$.
We note that
$\absState = \Base(\concState) \dagger \lstates{\proc}[\pc]$.
Let $\lstates{\proc}[\pc] = \st{\hat{L}_0,\hat{S}_0,B_0}$.
Let $\absState' = \Base(\concState) \dagger \st{\hat{L},\hat{S},B}$.
We must show $\inv(\concState',\absState')$.
The proof proceeds by case analysis according to the
local instruction that is executed to reach $\concState'$.
There are four parts of the invariant to check for each instruction:
type agreement, no memory leaks, no dangling references, and referential transparency.
The first two conditions are straightforward for all local instructions and are
therefore omitted from this presentation of the proof.

\paragraph{$\ao{\borrowlocCmd}{x}$.}
Suppose $\bcodes{\proc}(\pc) = {\ao{\borrowlocCmd}{x}}$ with $\lread{L}{x}=c$.
This instruction pushes a reference to $c$ on top of the operand stack.
The operational semantics give us
\[
\concState' = \st{\stackht{(\proc, \pc, L)}{P},\stackht{\rft{c}{[]}}{S},M}.
\]
The rule for $\ao{\borrowlocCmd}{x}$ shows
$\lread{\hat{L}_0}{x} = t$ for $t \in \valtype$,
$\hat{L} = \hat{L}_0$,
$\hat{S} = \stackht{\mut{t}}{\hat{S}_0}$, and
$B = \factor{B_0}{\psloc(0,x)}{\osloc(\len{\hat{S}_0})}$.
Thus, $B$ is derived from $B_0$ by
\begin{enumerate}
\item adding the edge $Borrow(\psloc(0,x),{\varepsilon},{\osloc(\len{\hat{S}_0})})$, and
\item replacing each edge $Borrow(\psloc(0,x),p,n)$ by the edge
$Borrow(\osloc(\len{\hat{S}_0}),p,n)$.
\end{enumerate}

\noindent {\em No dangling references.}
The only new position in $\abs{\concState'}$ is the new top of the operand stack
containing a mutable reference.
The new borrow edge $Borrow(\psloc(0,x),{\varepsilon},{\osloc(\len{\hat{S}})}$
incident on this position is realized.
Also, any realized borrow edge leaving $\psloc(0,x)$ that was moved to leave from
$\osloc(\len{\hat{S}})$ continues to be a realized edge.
Therefore the property holds for $\concState'$ and $\absState'$.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the new location $\osloc(\len{\hat{S}})$.

Let $m \neq \osloc(\len{\hat{S}})$ and $n \neq \osloc(\len{\hat{S}})$.
This case works because the factor operation is such that any realizable path
that went through $\psloc(0,x)$
now goes through both $\psloc(0,x)$ and $\osloc(\len{\hat{S}})$.

If $m=\osloc(\len{\hat{S}})$,
then $\concState(\psloc(0,x)) < \concState(n)$.
There is a realizable path in $\concState$ from $\psloc(0,x)$ to $n$ by induction.
This path can be transformed into a realizable path in $\concState'$
that goes through $\osloc(\len{\hat{S}})$.

If $n=\osloc(\len{\hat{S}})$,
then either $m = \psloc(0,x)$ or $\concState(m) = \concState'(m) = \concState'(n)$.
In the first case, the required path is simply the new $\varepsilon$-edge.
In the second case,
there is a realizable path in $\concState$ from $\psloc(0,x)$ to $m$ by induction.
This path can be transformed into a realizable path in $\concState'$
that goes through $\osloc(\len{\hat{S}})$.

\paragraph{$\ao{\borrowfieldCmd}{f,x}$.}
Suppose $\bcodes{\proc}(\pc) = \ao{\borrowfieldCmd}{f,x}$ with $\lread{L}{x} = \rft{c}{p}$.
There are two cases, based on whether $\lread{\hat{L}_0}{x} = \mut{\record{(f,t),\ldots}}$ or
$\lread{\hat{L}_0}{x} = \imm{\record{(f,t),\ldots}}$.
In both cases,
the instruction pushes a reference $\rft{c}{p::f}$ derived from
$\lread{L}{x}$ on top of the operand stack.
The operational semantics gives us
 \[
\concState' = \st{\stackht{(\proc, \pc, L)}{P},\;\stackht{\rft{c}{p::f}}{S},\;M}.
\]
However, the static analysis differs in the two cases.
We prove each case separately.

\noindent {\em Case 1.}
Suppose $\lread{\hat{L}_0}{x} = \mut{\record{(f,t),\ldots}}$ is a mutable reference.
The corresponding borrow-checker rule shows
$\hat{L} = \hat{L}_0$,
$\hat{S}= \stackht{\mut{t}}{\hat{S}_0}$, and
$B = \factorf{f}{B_0}{\psloc(0,x)}{\osloc(\len{\hat{S}})}$.
This borrow graph operation \emph{fails} and the bytecode program is rejected
if there is any edge labeled $\varepsilon$ or $*$
coming out of $\psloc(0,x)$ in $B_0$.
We therefore assume there is no such edge in $B_0$ and
derive $B$ from $B_0$ by
\begin{itemize}
\item Adding the edge $Borrow(\psloc(0,x),{f},{\osloc(\len{\hat{S}})}$, and
\item Replacing each edge $Borrow(\psloc(0,x),\concat{f}{p},n)$ by the edge $Borrow(\osloc(\len{\hat{S}},p,n)$.
\end{itemize}

\noindent {\em No dangling references.}
This proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the new location $\osloc(\len{\hat{S}})$.

If $m \neq \osloc(\len{\hat{S}})$ and $n \neq \osloc(\len{\hat{S}})$,
then the proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

If $m=\osloc(\len{\hat{S}})$, then $\concState(\psloc(0,x)) < \concState(n)$.
There is a realizable path in $\concState$ from $\psloc(0,x)$ to $n$ by induction.
Since there is no edge labeled $\varepsilon$ or $*$ out of $\psloc(0,x)$,
this path must follow one of the factored edges.
Therefore, this path can be transformed to go through $\osloc(\len{\hat{S}})$
in $\concState'$.

If $n=\osloc(\len{\hat{S}})$,
then $\concState(m) < \concState(\psloc(0,x))$
or $\concState(\psloc(0,x)) = \concState(m)$
or $\concState(\psloc(0,x)) < \concState(m)$.
In the first case,
there is a realizable path in $\concState$ from $m$ to $\psloc(0,x)$ by induction.
We can extend this path to $n$ by using the realizable edge from $\psloc(0,x)$ to
$\osloc(\len{\hat{S}})$.
In the second case,
there must be a realizable path either from $m$ to $\psloc(0,x)$ or from
$\psloc(0,x)$ to $m$ by induction.
Since there is no edge labeled $\varepsilon$ or $*$ out of $\psloc(0,x)$,
the realizable path must be from $m$ to $\psloc(0,x)$.
We can extend this path to $n$ by using the realizable edge from $\psloc(0,x)$ to
$\osloc(\len{\hat{S}})$.
In the third case, $\concState(m) = \concState'(m) = \concState'(n)$ and
there is a realizable path in $\concState$ from $\psloc(0,x)$
to $m$ by induction.
Since there is no edge labeled $\varepsilon$ or $*$ out of $\psloc(0,x)$,
this path must follow one of the factored edges.
Therefore, this path can be transformed to go through $\osloc(\len{\hat{S}})$
in $\concState'$.

\noindent {\em Case 2.}
Suppose $\lread{\hat{L}_0}{x} = \imm{\record{(f,t),\ldots}}$ is an immutable reference.
The corresponding borrow-checker rule shows
$\hat{L} = \hat{L}_0$,
$\hat{S}= \stackht{\imm{t}}{\hat{S}_0}$, and
$B = B_0 \cup \{\Borrow(\psloc(0,x),f,\osloc(\len{\hat{S}})\}$.

\noindent {\em No dangling references.}
This proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the new location $\osloc(\len{\hat{S}})$.

If $m \neq \osloc(\len{\hat{S}})$ and $n \neq \osloc(\len{\hat{S}})$,
then the proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

If $m=\osloc(\len{\hat{S}})$,
then $\concState(\psloc(0,x)) < \concState(n)$.
We get $\concState(n) \in \immreftype$ by induction.

If $n=\osloc(\len{\hat{S}})$,
then $\concState(m) < \concState(\psloc(0,x))$
or $\concState(m) = \concState(\psloc(0,x))$
or $\concState(\psloc(0,x)) < \concState(m)$.
In the first case, by induction (instantiating $m$ with $m$ and $n$ with $\psloc(0,x)$),
either $\concState(m) \in \immreftype$ or
$\concState(m) \not \in \immreftype$ and there is a realizable path in $\concState$ from
$m$ to $\psloc(0,x)$ which can be extended to a realizable path in $\concState'$ to $n$.
In the second case, by induction (instantiating $m$ with $\psloc(0,x)$ and $n$ with $m$),
either $\concState(m) \in \immreftype$ or
$\concState(m) \not \in \immreftype$ and there is a realizable path in $\concState$ from
$m$ to $\psloc(0,x)$ which can be extended to a realizable path in $\concState'$ to $n$.
In the third case, we get $\concState(m) \in \immreftype$ by induction.

\paragraph{$\ao{\movelocCmd}{x}$.}
Vertices in the borrow graph
are renamed from the old position of the moved value to its new position.
The new position does not appear as the source or target of any borrow
edge in the borrow graph.
Therefore, the new borrow graph is isomorphic to the old borrow graph.
Properties (No dangling references) and  Referential transparency) follow
from the fact that these properties held before this instruction was executed.

\paragraph{$\popCmd$.}
The analysis pops the top of the abstract operand stack and
eliminates the location corresponding to it using the
$\mathit{elim}$ operation on borrow graphs.
This operation eliminates location $u$ in $B_0$ as follows:
(1)~For every edge $\Borrow(a,p,u)$ coming into $u$ and edge $\Borrow(u,q,b)$
going out of $u$, add an edge $\Borrow(a,\concat{p}{q},b)$.
(2)~Delete all edges coming into and going out of $u$.
This ensures that all transitive borrow relationships
going through the reference that has been popped off the operand stack are
maintained,
preserving (No dangling references) and (Referential transparency) as a result.

\paragraph{$\ao{\storelocCmd}{x}$.}
The proof is a combination of the
proof for $\ao{\movelocCmd}{x}$ and $\popCmd$.

\paragraph{$\ao{\copylocCmd}{x}$.}
The proof is similar to $\ao{\borrowlocCmd}{x}$
in case the variable $x$ being copied is a reference.
Otherwise,
there is no change in the borrow graph and the proof is straightforward.

\paragraph{$\writerefCmd$.}
The proof is similar to $\popCmd$.

\paragraph{$\freezerefCmd$.}
The operational semantics gives us $\concState' = \concState$.
If the reference on top of the abstract operand stack in $\abs{\concState}$
is immutable, the local abstract state does not change and the proof is done.
Otherwise, the freezable mutable reference at the top of the abstract operand
stack is converted into an immutable reference.

\noindent {\em No dangling references.}
This proof is straightforward since there is no change in the borrow graph.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the location $\osloc(\len{\hat{S}}-1)$.

If $m \neq \osloc(\len{\hat{S}}-1)$ and $n \neq \osloc(\len{\hat{S}}-1)$,
then the proof is straightforward.

Suppose $m=\osloc(\len{\hat{S}}-1)$.
By induction, either
(1)~there is a path realizable in $\concState$ from $m$ to $n$, or
(2)$\concState(m) = \concState(n)$ and there is a path realizable
in $\concState$ from $n$ to $m$.
In the first case, the freezability of $m$ and Lemma~\ref{no-path-imm-to-mut}
indicate that $\absState(n) \in \immreftype$.
Since $\absState(n) = \absState'(n)$, we are done.
In the second case, we can reuse the path since $\concState = \concState'$.

Suppose $n=\osloc(\len{\hat{S}}-1)$.
By induction, either
(1)~$\absState(m) \not \in \immreftype$ and there is a path realizable
in $\concState$ from $m$ to $n$, or
(2)$\concState(m) = \concState(n)$ and there is a path realizable
in $\concState$ from $n$ to $m$.
In the first case, we can reuse the path since $\concState = \concState'$ and
$\absState(m) = \absState'(m)$.
In the second case, the freezability of $n$ and Lemma~\ref{no-path-imm-to-mut}
indicate that $\absState(m) \in \immreftype$.
Since $\absState(m) = \absState'(m)$, we are done.

\paragraph{$\readrefCmd$.}
The proof is similar to $\popCmd$.

We omit discussion of $\packCmd$, $\unpackCmd$, and $\stackopCmd$
since these instructions do not perform any reference-related operations.
\end{proof}


==> revised-borrow-checker-rules.tex <==
\begin{figure*}
\begin{centerframe}

\pcrule[]
  {
    x \not \in 0..\len{\ins{\proc}} \sep
    x \in \dom{\hat{L}}\sep
    \lread{\hat{L}}{x} \in \valtype\Rightarrow
    \Unborrowed(B,\psloc(0,x))\sep
    B' = \rename{B}{\psloc(0,x),\osloc(0,\len{\hat{S}})}
  }
  {\proc,\ao{\movelocCmd}{x}}
  {\st{\hat{L},\hat{S},B}}
  {\st{\mdel{\hat{L}}{x},\stackht{\lread{\hat{L}}{x}}{\hat{S}},B'}}
  \bigskip

\pcrule[]
  {
    B'= \elim{B}{\osloc(\len{\hat{S}})}
  }
  {\proc,\popCmd}
  {\st{\hat{L},\stackht{\_}{\hat{S}},B}}
  {\st{\hat{L},\hat{S},B'}}
 \hspace{4mm}
   %\bigskip
\pcrule[Ref]
  {
    x \not \in 0..\len{\ins{\proc}} \sep
    \lread{\hat{L}}{x} \in \reftype\sep
    B' = \rename{\elim{B}{\psloc(0,x)}}{\osloc(\len{\hat{S}}),\psloc(0,x)}
  }
  {\proc,\ao{\storelocCmd}{x}}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  {\st{\lset{\hat{L}}{x}{t},\hat{S},B'}}
  \bigskip

\pcrule[Val]
  {
    x \not \in 0..\len{\ins{\proc}} \sep
    x\not\in\dom{\hat{L}} \vee \lread{\hat{L}}{x} \in \valtype \\\\
    \Unborrowed(B,\psloc(0,x)) \sep
    B' = \rename{B}{\osloc(\len{\hat{S}}),\psloc(0,x)}
  }
  {\proc,\ao{\storelocCmd}{x}}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  {\st{\lset{\hat{L}}{x}{t},\hat{S},B}}
  \hspace{8mm}
\pcrule[]
  {
    x \in \dom{\hat{L}}\sep
    \lread{\hat{L}}{x} = t \sep t \in \valtype \\\\
    B' = \factor{B}{\psloc(0,x)}{\osloc(\len{\hat{S}})}
  }
  {\proc,\ao{\borrowlocCmd}{x}}
  {\st{\hat{L},\hat{S},B}}
  {\st{\hat{L},\stackht{\mut{t}}{\hat{S}},B'}}
  \bigskip

\pcrule[Mut]
  {
    x \in \dom{\hat{L}}\sep
    \lread{\hat{L}}{x} = \mut{\record{(f,t),\ldots}} \\\\
    B' = \factorf{f}{B}{\psloc(0,x)}{\osloc(\len{\hat{S}})}
  }
  {\proc,\ao{\borrowfieldCmd}{f,x}}
  {\st{\hat{L},\hat{S},B}}
  {\st{\hat{L},\stackht{\mut{t}}{\hat{S}},B'}}
  \hspace{7mm}
\pcrule[Immut]
  {
    x \in \dom{\hat{L}}\sep
    \lread{\hat{L}}{x} = \imm{\record{(f,t),\ldots}} \\\\
    B' = B \cup \{\Borrow(\psloc(0,x),f,\osloc(\len{\hat{S}})\}
  }
  {\proc,\ao{\borrowfieldCmd}{f,x}}
  {\st{\hat{L},\hat{S},B}}
  {\st{\hat{L},\stackht{\imm{t}}{\hat{S}},B'}}
  \bigskip

\pcrule[]
  {
    x \in \dom{\hat{L}}\sep
    B' = \ite{\lread{\hat{L}}{x} \in \reftype}{\factor{B}{\psloc(0,x)}{\osloc(\len{\hat{S}})}}{B}
  }
  {\proc,\ao{\copylocCmd}{x}}
  {\st{\hat{L},\hat{S},B}}
  {\st{\hat{L},\stackht{\lread{\hat{L}}{x}}{\hat{S}},B'}}
  \vspace{2mm}

\pcrule[]
  {
    \Borrow(\osloc(\len{\hat{S}}), \_, \_) \not \in B\sep
    B' = \elim{B}{\osloc(\len{\hat{S}})}
  }
  {\proc,\writerefCmd}
  {\st{\hat{L},\stackht{t}{\stackht{\mut{t}}{\hat{S}}},B}}
  {\st{\hat{L},\hat{S},B'}}
  \bigskip

\pcrule[]
  {
    t = \imm{t'} \vee t = \mut{t'}\\\\
    \forall n.\ \Borrow(\osloc(\len{\hat{S}}), \_, n) \in B \Rightarrow \st{\hat{L},\hat{S}}[n] \in \immreftype
  }
  {\proc,\freezerefCmd}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  {\st{\hat{L},\stackht{\imm{t'}}{\hat{S}},B}}
  \hspace{5mm}
\pcrule[]
  {
    t = \imm{t'} \vee t = \mut{t'}\sep
    B' = \elim{B}{\osloc(\len{\hat{S}})} \\\\
    \forall n.\ \Borrow(\osloc(\len{\hat{S}}), \_, n) \in B \Rightarrow \st{\hat{L},\hat{S}}[n] \in \immreftype
  }
  {\proc,\readrefCmd}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  {\st{\hat{L},\stackht{t'}{\hat{S}},B'}}
  \bigskip

\pcrule[]
  {
    \overline{t} = [t_1,\ldots,t_n]\sep
    t = \record{(f_{i},t_{i})\mid 1 \leq i \leq n}
  }
  {\proc,\ao{\packCmd}{t}}
  {\st{\hat{L},\stackht{\overline{t}}{\hat{S}},B}}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  \hspace{5mm}
\pcrule[]
  {
    \overline{t} = [t_1,\ldots,t_n]\sep
    t = \record{(f_{i},t_{i})\mid 1 \leq i \leq n}
  }
  {\proc,\unpackCmd}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  {\st{\hat{L},\stackht{\overline{t}}{\hat{S}},B}}
  \hspace{5mm}
\pcrule[]
  {
    \typeof{\stackop}{\overline{t} \rightarrow t}
  }
  {\proc,\stackopCmd}
  {\st{\hat{L},\stackht{\overline{t}}{\hat{S}},B}}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  \bigskip

\pcrule[]
  {
    \is = 0..\len{\ins{\proc'}} \sep
    \os = 0..\len{\outs{\proc'}} \\\\
    \forall i \in \is.\ \ins{\proc'}[i] \in \mutreftype \Rightarrow
    \Borrow(\osloc(\len{\hat{S}}+i),\_,\_) \not \in B\\\\
    B_1 = \rename{B}{\{
                      i \in \is \mid
                      (\osloc(\len{\hat{S}}+i), \psloc(1,i))
                  \}}\\\\
    B_2 = \extend{B_1}{\{
                        \psloc(1,i) \mid
                        i \in \is \wedge \ins{\proc'}[i] \in \mutreftype
                    \}}{\{
                        \osloc(\len{\hat{S}}+i) \mid i \in \os \wedge \outs{\proc'}[i] \in \reftype
                    \}}\\\\
    B_3 = \extend{B_2}{\{
                          \psloc(1,i) \mid
                          i \in \is \wedge \ins{\proc'}[i] \in \immreftype
                      \}}{\{
                          \osloc(\len{\hat{S}}+i) \mid
                          i \in \os \wedge \outs{\proc'}[i] \in \immreftype
                      \}}\\\\
    B' = \elim{B_3}{\{ \psloc(1,i) \mid i \in \is \}}
  }
  {\proc,\ao{\callCmd}{\proc'}}
  {\st{\hat{L},\stackht{\reverse{\ins{\proc'}}}{\hat{S}},B}}
  {\st{\hat{L},\stackht{\reverse{\outs{\proc'}}}{\hat{S}},B'}}
  \bigskip

\pcrule[]
  {
    \hat{L} = \ins{\proc} \sep \forall x \in \dom{\hat{L}}.\ \lread{\hat{L}}{x} \in \valtype \Rightarrow \Borrow(\psloc(0,x),\_,\_) \not \in B\\\\
    \hat{S} = \reverse{\outs{\proc}}\sep
    \forall i \in \dom{\hat{S}}.\ \hat{S}[i] \in \mutreftype \Rightarrow \Borrow(\osloc(i),\_,\_) \not \in B
  }
  {\proc,\returnCmd}
  {\st{\hat{L},\hat{S},B}}
  {\st{\hat{L},\hat{S},B}}
  \hspace{3mm}
\pcrule[]
  {
    t = \booleantype
  }
  {\proc,\ao{\branchCmd}{\pc_1,\pc_2}}
  {\st{\hat{L},\stackht{t}{\hat{S}},B}}
  {\st{\hat{L},\hat{S},B}}
  \bigskip

\label{fig:rules-borrow-checker}
\end{centerframe}
\end{figure*}


==> revised-borrow-checker.tex <==
\setlength{\abovedisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}

\section*{Revised Borrow Checker}
\paragraph{Positions}
In specifying the types of local variables, the type of entries on the operand stack,
and relationships between locations and references stored in them, 
we use two forms of \emph{position,}
written $\psloc(x, y)$ and $\osloc(x,y)$ for non-negative integers $x$ and $y$.

For concrete state $\concState = \st{P,M}$,  the position 
$\psloc(x, y)$ refers to the $y$-th local variable in the $x$-th call frame of the stack and
$\osloc(x,y)$ refers to the $y$-th operand-stack position in the $x$-th call frame of the stack.

We let $\dom{P}$ be the set of local variable and operand-stack positions that are used in $P$,  i.e.,
$\psloc(x, y)$ for $x$ less than the total number of call frames in $P$ and
$y$ less than the number of local variables in the $x$th frame,  
\emph{counting from the bottom of the call stack,} or
$\osloc(x, y)$ with $x$ less than the total number of call frames in $P$ and
$y$ less than the  height of the operand  in the $x$th frame.
If $\concState = \st{P,M}$,  then $\dom{\concState}= \dom{P}$.

\paragraph{Abstract state}
An \emph{abstract state} $\absState$ is represented by an 
\textit{abstract call stack}  $\hat{P} = \hat{F}_n \cons \ldots \cons \hat{F}_0$ where each 
\textit{abstract call-stack frame},  
$\hat{F}_i = \st{ \proc,\pc, L,S,B}$ comprises
a procedure name \proc,
a program counter $\pc$, 
a partial map $\hat{L}$ from variables to $\type$,
a list $\hat{S}$ of types,
and a \textit{borrow graph} $B$.
Absolute positions in the local variable map $\hat{L}$ and operand-stack types $\hat{S}$
are defined in the same ways as for a concrete call-stack.
We write $\dom{\hat{P}}$ for the set of local variable and operand-stack positions in $\hat{P}$.

A borrow graph  $B$  is a labeled directed graph whose 
nodes are positions; each edge is labeled by a path.
We write $\Borrow(x,p,y)$ for the \emph{borrow edge} from node $x$ to node $y$ with label $p$.
If $B$ is the borrow graph of a frame $\hat{F}_i $,
then positions $\psloc(x, y)$ and $\osloc(x,y)$ are interpreted as \textit{relative positions}
that are relative to the height $i$ of this frame in the call stack.
Specifically,  a relative position $\psloc(x, y)$ in borrow graph $B$ of frame at height $i$
refers to absolute position $\psloc(x+i, y)$,  and similarly for $\osloc(x,y)$.

An \textit{abstract call stack}  $\hat{P} = \hat{F}_n \cons \ldots \cons \hat{F}_0$
defines a borrow graph $BG(\hat{P})$ whose nodes are absolute positions. 
The graph $B = BG(\hat{P})$ has edge
$\Borrow(\psloc(x+i, y),p,\psloc(u+i, v)) \in B$
for each
$\Borrow(\psloc(x, y),p,\psloc(u, v)) \in B_i$ at stack level $i$,
and similarly for all other combinations of $\psloc(x, y)$ and $\osloc(x,y)$
used as relative positions. 
An abstract call stack  $\hat{P}$ is considered \textit{well-formed} only
if every absolute position produced in this way is in $\dom{\hat{P}}$.

\paragraph{States as partial maps.}
Concrete and abstract states each induce a partial function from call-stack positions to values or types.
Specifically,  if $\concState$ is a concrete state,  then for any call-stack position in  $\dom{\concState}$, we write
$\absState(\psloc(x, y))$ for the value of the $y$-th local variable in the $x$-th call frame of the stack and
$\absState(\osloc(x,y))$ for the value  in $y$-th operand-stack position in the $x$-th call frame of the stack.
We similarly treat any abstract state $\absState$ as a partial map from call-stack positions 
$\dom{\absState}$ to types,  with 
$\absState(\psloc(x, y))$ the type given to the $y$-th local variable in the $x$-th call frame of the stack and
$\absState(\osloc(x,y))$ the type in $y$-th operand-stack position in the $x$-th call frame of the stack.

\paragraph{Type and shape matching}
Concrete state $\concState = \st{P,M}$ and
abstract state $\absState$ are {\em shape-matching} if
$\dom{\concState} = \dom{\absState}$,
and for all $i  \leq \len{P}$,  we have $P[i].\proc = \hat{P}[i].\proc$ and $P[i].\ell = \hat{P}[i].\ell$.
Shape-matching states $\concState$  and $\absState$ are
further \emph{type-matching} if for all  $i \in \dom{\concState} = \dom{\absState}$
in the identical sets of positions,  we have $\typeof{\concState(i)}{\absState(i)}$.

\paragraph{Borrow graph intuition}
A borrow graph in an abstract state expresses borrow relationships between references
in any corresponding concrete state.
If concrete state $\concState$ and
abstract state $\absState$ are shape-matching and type-matching,
with positions $x,y \in  \dom{\concState} = \dom{\absState}$,
then an edge $\Borrow(x,p,y)$ in $\absState$ indicates that in $\concState$,  the reference
$x.p$ \textit{is borrowed by} $y$.
If $p$ is fixed, the reference in $\concState$ at position $y$ has jurisdiction
over $m.p$, where $m$ is the reference or concrete location at position $x$
in the $\concState$.
If $p$ is extensible, then $x.q$ is borrowed by $y$ for some extension $q$ of $p$.

\paragraph{Realized edge}
For shape-matching $\concState = \st{P,M}$ and $\absState$,
a borrow edge $\Borrow(m,p,n)$ in $BG(\absState)$
is \emph{realized in} $\concState$ if the path $p$ leads from $\concState(m)$ to $\concState(n)$,
optionally involving additional field selections if $p$ ends in $*$.
More precisely, we say this graph edge is realized if either
\begin{enumerate}
\item $\concState(m) = c$, $\concState(n) = \rft{c}{q'}$, and path $p$ matches $q'$, or
\item $\concState(m) = \rft{c}{q}$, $\concState(n) = \rft{c}{q'}$, and $q.p$ matches $q'$.
\end{enumerate}
Note that the two conditions express the same basic relationship if we identify $c$ and $ \rft{c}{\varepsilon}$.

We write $\rft{c}{p} \leq \rft{d}{q}$ if $c = d$ and $p \leq q$.
We extend $\leq$ so that $c \leq \rft{c}{p}$ for any~$p$.  
\jm{where to put this best?}

\paragraph{Borrow graph subsumption}
An edge $\Borrow(x, p, y)$ is {\em subsumed} by edge $\Borrow(x,q,y)$ if
either $p=q$ or $q = r*$ and $r \leq p$.
If $G$ and $H$ are borrow graphs, we write $G \below H$,
if every edge $\Borrow(x,p,y)$ in $G$ is subsumed by some edge $\Borrow(x,q,y)$ in $H$.
Note that this definition allows additional edges in $H$ that are not implied by edges in $G$.
Semantically, if $G \below H$, then $G$ imposes every restriction on concrete execution that is
expressed by $H$, and possibly additional restrictions.
As a result, we will see that every state that satisfies $G$ also satisfies $H$.


\paragraph{Parameter passing and return}
Before a procedure call,  the bytecode program is assumed to contain
instructions that put the parameters for the call on the top of the operand stack.
As part of the \callCmd command,  these parameter values are 
removed from the local operand stack of the caller 
and placed on the local operand stack of the callee.
For this reason,  procedure execution begins with stack entries whose types 
are the declared types of the formal parameters; 
we manage this by setting types in the abstract state accordingly.

When the procedure returns,  the return value is transferred from the returning procedure's 
operand stack to the operand stack of the procedure that called it. 
This is similarly managed in the static analysis by giving the top value in the 
callee stack the type of the procedure return value.

We use the notation $\ins{\proc}$ for the list of parameter types of $\proc$
and $\outs{\proc}$ for the return type, both as specified in the procedure declaration.

\paragraph{Abstract semantics of instructions (= Type propagation)}
The borrow checker analyzes each procedure independently,
in a manner that is characterized by a set of 
rules for propagating type and borrow relationships through individual instructions.
These rules are applied successively to each instruction in the procedure,
beginning with an abstract state characterizing the local variables and parameters
passed into the procedure when it is first called. 
The data structure used to characterize the static information is  
an extended abstract call-stack frame, as defined above,
although the procedure name and program counter do not affect
the semantics of an instruction.

The rules for type propagation of local instructions (\S \ref{sec:propagation})
%(\Cref{fig:rules-borrow-checker})
operate over a local abstract state $\st{\hat{L},\hat{S},B}$,
where $\hat{L}$ maps local variables to types,
$\hat{S}$ is a list of types for the values and references in the operand stack,
and $B$ is a borrow graph over positions in $\hat{L}$ and $\hat{S}$.
We write $\ls.B$ for the borrow-graph component of the local state,
and similarly $\ls.L$ and $\ls.S$.  \jm{check consistent notation}

An abstract local state $\ls$ is {\em well-formed} for $\proc$ if
(1)~every input location of $\proc$ is in $\dom{\ls}$,
(2)~$\ls.B$ is a directed acyclic graph, and
(3)~for all $\Borrow(x,\_,y) \in \ls.B$, we have $x,y \in \dom{\ls}$, and
$y$ is not an input location of $\proc$.

The propagation on local abstract states (\S \ref{sec:propagation}) uses judgments of the form
$
\proc,\op \vdash \st{\hat{L},\hat{S},B} \rightarrow \st{\hat{L}',\hat{S}',B'}
$
indicating that procedure $\proc$ executing instruction $\op$
from $\st{\hat{L},\hat{S},B}$ results in $\st{\hat{L}',\hat{S}',B'}$.
These rules are designed to ensure that if $\st{\hat{L},\hat{S},B}$ is well-formed for
$\proc$, then $\st{\hat{L}',\hat{S}',B'}$ is also well-formed for $\proc$.

Extending to the partial ordering $\below$ on borrow graphs to abstract states,
we write $\st{\hat{L},\hat{S},B} \below \st{\hat{L}',\hat{S}',B'}$ if
$\hat{L} = \hat{L}'$, $\hat{S} = \hat{S}'$, and $B \below B'$.
It will follow from the properties of $\below$ on borrow graphs that
every concrete local state meeting the conditions imposed by $\st{\hat{L},\hat{S},B}$ 
also meets those imposed by $\st{\hat{L'},\hat{S'},B'}$.

\paragraph{Well-typed programs}
%Our analysis requires that each procedure $\proc$ has the following annotations:
%(1)~a sequence of input types $\ins{\proc}$,
%(2)~a sequence of output types $\outs{\proc}$,
%(3)~for each offset $i \in 0..\len{\bcodes{\proc}}$, an abstract local state $\lstates{\proc}[i]$
%that is well-formed for $\proc$.
In proving the soundness of the borrow checker,  we assume the program is annotated
with an  appropriate  abstract state for entry to each instruction.
Specifically,  for each procedure $\proc$,  we assume there is a given 
abstract local state $\lstates{\proc}[i]$ for each offset $i \in 0..\len{\bcodes{\proc}}$.
To be well-typed,  each abstract state must be well-formed for the procedure 
in which it occurs and must satisfy two additional conditions,
one involving the initial input conditions and the other involving control flow.

\textit{Initial state condition.}
Because \jm{ fix this},  we require that$\st{\ins{\proc},[],\{\}} = \lstates{\proc}[0]$,
meaning  \ldots (on procedure entry,   the operand stack and borrow graph are empty;
possibly  not correct because of parameter passing on the operand stack)

Second, the abstract state annotations must reflect the control flow of the program.  
To state this, we let  $\Next{\proc}[i]$ be the set of program counters
to which control transfer is possible after executing instruction at position $i$,
specifically
\[
\begin{array}{llll}
  \Next{\proc}[i] & = & \{\}, & \ifcmd\ \bcodes{\proc}[i] = \returnCmd \\
                  &   & \{\pc_1, \pc_2\}, & \ifcmd\ \bcodes{\proc}[i] = \ao{\branchCmd}{\pc_1, \pc_2} \\
                  &   & \{\pc+1\}, & \mathit{otherwise}
\end{array}
\]

\textit{Control flow condition.}
For all for all $i \in \dom{\bcodes{\proc}}$,   there must be an abstract state with
$\proc,\bcodes{\proc}[i] \vdash \lstates{\proc}[i] \rightarrow \st{\hat{L},\hat{S},B}$
according to the propagation rules and 
$\st{\hat{L},\hat{S},B} \below \lstates{\proc}[j]$ for all $j \in \Next{\proc}[i]$.
In other words,  any conditions expressed in the abstract state propagation rules must be
met and the abstract state produced by applying the propagation rules 
must be $\below$ the annotation of any next program state.
We do not require equality because there may be more than
one control path for reaching the next instruction and the 
borrow checking algorithm may therefore select some 
abstract state that is $\abve$ all of them.

A program $\program$ is {\em well-typed} 
if the initial state condition and the control flow condition 
above are met for  all $\proc \in \dom{\program}$.

\paragraph{State abstraction function }
We can combine program annotations,  which give a local abstract state for each program point,
with a concrete state that has a stack of program points, to produce an abstract state.
This abstraction function has the property that
as a concrete execution steps through concrete states, 
abstract execution steps through the corresponding abstract states.

Given any concrete state  $\concState =\st{P, M}$ for a well-typed program $\program$,
we define the abstract state $\abs{P} = \hat{P}$ 
by induction on the height of $P$.

If the concrete call-stack $P = [\;]$ is the empty list,  
then $\abs{P} = [\;]$ is empty.

If the concrete call-stack is $\st{\proc,\pc, L,S}\cons P$,
the corresponding abstract call-stack is 
\[
 \st{\proc,\pc,, \hat{L},\hat{S},B}\cons \abs{P}
\]
where
$\st{\hat{L},\hat{S},B} =  \lstates{\proc_0}[\pc_0]$
is the type annotation for program point $\pc$ in the  procedure $\proc$.
For $\concState =\st{P, M}$,  we let $\abs{\concState}=\abs{P} $.

\section*{Borrow Checker Invariants}

We use the abstraction function to prove critical invariants
about executions of well-typed programs.
These invariants establishes four properties: type agreement,  no memory leaks,
no dangling references, and referential transparency.
We combine these invariants as a predicate $\inv(\concState,\absState)$
over a concrete state $\concState$ and an abstract state $\absState$.

\begin{manualtheorem}{1}
\label{type-sound-thm}
    Let program $\program$ be well-typed.
    If $\concState$ is a concrete state with $\inv(\concState,\abs{\concState})$
    and $\program \vdash \concState \rightarrow \concState'$,
    then $\inv(\concState',\abs{\concState'})$.
\end{manualtheorem}

A corollary is that if $\program$ starts execution in
a concrete state $\concState_0$ such that $\inv(\concState_0,\abs{\concState_0})$ holds,
then $\inv(\concState,\abs{\concState})$ holds for all states
reachable from~$\concState_0$.
Any initial state $\concState_0$ of $\program$ is of the form
$\st{(\proc,0,\overline{x}),[],\{\}}$ representing the beginning of
a transaction that invokes $\proc$ with inputs $\overline{x}$ comprising only values
(no references), empty operand stack, and empty memory.
It is easy to see that $\inv(\concState_0,\abs{\concState_0})$ holds
if $\program$ is well-typed.

We define $\inv$ as the conjunction of four predicates,
$\inva$, $\invb$, $\invc$, $\invd$, described below.

\paragraph{Type Agreement} 
\hfill\\
\noindent
$\inva(\concState,\absState):$
$\concState$ and $\absState$ are shape-matching and type-matching.

\paragraph{No Memory Leaks}
The following invariant indicates that
(1)~every local variable on the call stack of $\concState$ contains a different location, and
(2)~locations are not leaked, i.e., $\concState.M$ does not contain any location
not present in a local variable.

\hfill\\
\noindent
$\invb(\concState,\absState):$
The relation
$\{ (n,\concState(n)) \mid n \in \dom{\absState} \wedge \concState(n) \in \cl \}$
is a bijection from its domain to $\dom{\concState.M}$.

\jm{Since $\dom{\absState}  = \dom{\concState}$,  it looks like this can be stated as a property
of $\concState$ without referring to $\absState$.
Does this property depend on the borrow checker?}

\paragraph{No Dangling References}
The following invariant allows us to conclude that every reference is rooted
in a memory location present in some local variable on the call stack.

\hfill\\
\noindent
$\invc(\concState,\absState):$
\begin{enumerate}
\item $BG(\absState)$ is acyclic.
% \sq{This conjunct may not be needed but a weaker conjunct that just prohibits
% incoming borrow edges may be needed to ensure hygiene of rename applications
% and to ensure that certain eliminations are not needed, e.g. the elimination
% of the written value in WriteRef.}
%  \item For all $n \in \dom{\absState}$ such that $\absState(n) \in \valtype$,
%  either $n = \psloc(\_,\_)$ and n has no incoming edges or
%  $n = \osloc(\_)$ and $n$ has no incident edges.
\item
For all $n \in \dom{\absState}$ such that $\absState(n) \in \valtype$,
there is no borrow edge in $BG(\absState)$ coming into $n$.
\item
For all $n \in \dom{\absState}$ such that $\absState(n) \in \reftype$,
there is a borrow edge in $BG(\absState)$ coming into $n$ that is realized in $\concState$.
\end{enumerate}

\paragraph{Referential Transparency}
The following invariant indicates that the absence of borrow edges out of an
abstract location containing a value or a mutable reference
guarantees that mutation via that abstract location,
either of the stored value or the value pointed to by the mutable reference,
will not invalidate any live reference.

\hfill\\
\noindent
$\invd(\concState,\absState):$
For any distinct $m,n\in\dom{\absState}$ such that
$\absState(n) \in \reftype$ and $\concState(m) \leq \concState(n)$,
one of the following hold:
\begin{enumerate}
\item
$\absState(m) \in \immreftype$ and $\absState(n) \in \immreftype$.
\item
$\absState(m) \not \in \immreftype$
and there is a path in $BG(\absState)$ from $m$ to $n$
comprising realized edges in $\concState$.
\item
% $\absState(n) \in \mutreftype$,
% The above conjunct was present in the next condition.
% I was able to convince myself that removing it leaves InvD semantically unchanged.
$\concState(m) = \concState(n)$
and there is a path in $BG(\absState)$ from $n$ to $m$
comprising realized edges in $\concState$.
\end{enumerate}

The following lemma  states an important
and useful fact connecting borrow graphs and reference types.
\begin{manuallemma}{0}
  \label{no-path-imm-to-mut}
  Suppose $\absState = \abs{\concState}$ and
  $\invd(\concState,\absState)$.
  If $m,n \in \dom{\absState}$ are distinct, $\absState(n) \in \mutreftype$,
  and there is a path in $BG(\absState)$ realizable in $\concState$ from $m$ to $n$,
  then $\absState(m) \not \in \immreftype$.
\end{manuallemma}

\begin{proof}[Proof of Lemma \ref{no-path-imm-to-mut}]
If there is a path in $B=BG(\absState)$ realizable in $\concState$ from $m$ to $n$,
then $\concState(m) \leq \concState(n)$.
We know that $\absState(n) \not \in \immreftype$.
We also know that since the borrow graph in $\absState$ is acyclic,
there is no path in it from $n$ to $m$.
The definition of referential transparency property expressed in $\invd$ allows us to conclude
that $\absState(m) \not \in \immreftype$.
\end{proof}

\subsection{Propagating Local Abstract States}
\label{sec:propagation}

\input{revised-borrow-checker-rules}

Having explained the overall structure of our soundness
argument, we now provide intuition for type propagation
on local abstract states.
The rule for operation $\op$ derives a judgment of the form
$
\proc,\op \vdash \st{\hat{L},\hat{S},B} \rightarrow \st{\hat{L}',\hat{S}',B'}
$
if certain conditions are satisfied.
These conditions include availability of appropriately-typed
values in $\hat{L}$ or $\hat{S}$ and absence of certain edges in
the borrow graph $B$.
The state transformation adds or removes a variable-to-type binding in $\hat{L}$,
pushes or pops types in $\hat{S}$, and adds or removes edges in $B$.
The rules for \movelocCmd and \storelocCmd also prevent an input of procedure $\proc$
from being moved or overwritten
to enable accurate tracking of transitive borrow relationships across a procedure call.

\paragraph{Operations on borrow graphs}
There are six operations on borrow graphs and two queries.

%\begin{enumerate}%[\leftmargin=0em]
%\item
(1)\quad
The operation $\rename{B}{u,v}$ replaces every edge $\Borrow(u,p,w) \in B$ with $\Borrow(v,p,w)$,
for all $w$.
This is used when position $u$ is eliminated and $v$ is created,
such as when a local variable is eliminated and its value pushed onto the operand stack.
In the case the second argument is a set,  $\rename{B}{\{(u_i,v_i)\mid i \in \is\}}$
replaces each $\Borrow(u_i,p,w)$ with $\Borrow(v_i,p,w)$, for all $w$.

%\item
(2)\quad
The operation $\factor{B}{u}{v}$ creates a new borrow graph by
replacing each edge $\Borrow(u,p,w)$ going out of $u$ 
by $\Borrow(v,p,w)$ going out of $v$ and adding a new edge $\Borrow(u,\varepsilon,v)$.
The node $u$ may have borrow edges incident in $B$ but $v$ may not.

%\item
(3)\quad
The operation $\mathit{factor}_f$ a is similar to $\mathit{factor}$.
It is a partial operation and may fail.
If there is no edge labeled $\varepsilon$ or $*$ coming out of $u$ in $B$,  then $\factor{B}{u}{v}$ succeeds 
and replaces each edge of the form $\Borrow(u,\concat{f}{p},a)$ by $\Borrow(v,p,a)$.
The operation also adds an edge $\Borrow(u,f,v)$.

%\item
(4)\quad
The operation $B \cup \Borrow(u,p,v)$ adds the edge $\Borrow(u,p,v)$,  if it is not already present.

%\item
(5)\quad
The operation $\extend{B}{\us}{\vs}$ is applicable to sets $\us$ and $\vs$ of positions,
where there may be borrow edges incident on locations in $\us$ but no borrow edges incident on
locations in $\vs$.
The result adds an edge $\Borrow(u,*,v)$ to $B$ for every $u \in \us$ and $v \in \vs$.

%\item
(6)\quad
The operation $\elim{B}{u}$ creates a new borrow graph by eliminating location $u$ in $B$ as follows:
(1)~For every edge $\Borrow(a,p,u)$ coming into $u$ and edge $\Borrow(u,q,b)$
going out of $u$,  add an edge $\Borrow(a,\concat{p}{q},b)$.
(2)~Delete all edges coming into and going out of $u$.

%\item 
(7)\quad
The predicate $\Unborrowed(B,u)$ is true if there are no 
outgoing borrow edges from $u$ in $B$.

%\item
(8)\quad
The set $\Borrowed(B,u)$ is the set of all $v$ borrowed from $u$ in $B$.
\jm{Is this set of $v$ with $\Borrow(u,p,v)$ for all $p$? Or just $\varepsilon$? Or any path?}
USED IN ``The rules for $\freezerefCmd$ and $\readrefCmd$ both check that the reference
operand at the top of the stack is {\em freezable}, i.e., all borrowed references
from it are immutable.''
%\end{enumerate}

\paragraph{Rules for instructions}
The rule for $\ao{\movelocCmd}{x}$ moves the type of variable $x$ to the top of
operand stack.
The rule checks that $x$ is available in $\hat{L}$
and there are no outgoing borrow edges from $\psloc(0,x)$, 
the abstract location of $x$,  in case $x$ is a value.
The rule also renames the old position of the moved value in the borrow graph to its new position.

The rule for $\popCmd$ pops the top of the operand stack and
eliminates the location corresponding to it using a new operation $\mathit{elim}$.
\jm{}
The definition of $\elim{B}{u}$ ensures that all transitive borrow relationships
going through the reference at the top of the operand stack are maintained even
when the top is popped.

The two rules for $\ao{\storelocCmd}{x}$ use a combination of the techniques introduced
for handling $\ao{\movelocCmd}{x}$ and $\popCmd$.
If $x$ is available in the local store and is a reference type,
$\psloc(0,x)$ is eliminated in the borrow graph.
If $x$ is available in the local store and is a value type,
then it is checked that there are no borrow edges going out of $\psloc(0,x)$.
In both cases, the position for the previous top of stack is renamed to $\psloc(0,x)$
since it is being moved into variable $x$.

The rule for $\ao{\borrowlocCmd}{x}$ uses the operation $\mathit{factor}$.
\jm{explain}
This operation ensures that borrows from $u$ are propagated to $v$.

The first rule for $\ao{\borrowfieldCmd}{f,x}$ addresses the case when
the source reference is mutable and creates a mutable borrow from it.
This rule uses $\mathit{factor}_f$,  which
 succeeds if there is no edge labeled $\varepsilon$ or $*$ coming out of $u$
in $B$,  converting each edge of the form $\Borrow(u,\concat{f}{p},a)$ to $\Borrow(v,p,a)$
and adding the edge $\Borrow(u,f,v)$.
This rule ensures that any borrows from variable $x$ along the field $f$ are
instead borrows from the new reference pushed on the operand stack which is itself
borrowed from $x$.

The second rule for $\ao{\borrowfieldCmd}{f,x}$ addresses the case when
the source reference is immutable and creates an immutable borrow from it.
This rule simply adds a borrow edge labeled $f$ between the source reference
and the new reference.

The rule for $\ao{\copylocCmd}{x}$ is similar to $\ao{\borrowlocCmd}{x}$
in case the variable $x$ being copied is a reference.
The rule for $\writerefCmd$ checks that the target reference does not have
any borrow edges coming out of it.
The rules for $\freezerefCmd$ and $\readrefCmd$ both check that the reference
operand at the top of the stack is {\em freezable}, i.e., all borrowed references
from it are immutable.
If a mutable reference is freezable, it is safe to convert it into an immutable reference.

For space reasons, we skip over the rules for $\packCmd$, $\unpackCmd$,
and $\stackopCmd$
which do not perform any reference-related operations.
\jm{Add explanation of these now?}

The rule for $\ao{\callCmd}{\proc'}$ can be understood as a sequence of simple steps.
First,  it checks that no mutable reference being passed to $\proc'$ is borrowed.
Second,  it renames the call arguments present on the operand stack to the corresponding
locals in the next frame to simulate the call (see definition of $B_1$).
Third,  it simulates the return from the call by adding borrow edges from input
reference parameters to output references returned by the call (see definition of
$B_2$ and $B_3$) and eliminating the locals in the callee frame (see definition of
$B'$).
The definitions of $B_2$ and $B_3$ use the $\mathit{extend}$ operation
and applies $\mathit{elim}$ to a set of locations to eliminate each of them from the borrow graph.

The rule for $\returnCmd$ checks that no local of value type is borrowed,
the contents of the operand stack matches the output signature of $\proc$,
and no output that is a mutable reference is borrowed.
This ensures that returned references are valid and the caller's expectations for borrow relationships are sound.
%These checks ensure that any returned reference is valid and the caller receives a
%sound model of borrow relationships among returned references.


==> revised-proof.tex <==
\newcommand{\halfstep}{\rightharpoonup}
\newcommand{\Base}{\mathit{Base}}
\newcommand{\hole}{\square}

\section*{Soundness proof}

We prove soundness of the borrow checker (Theorem \ref{type-sound-thm})
by showing that the inductive invariant between concrete and abstract states
is preserved by execution of any well-typed program.

The proof of Theorem \ref{type-sound-thm} is decomposed into several lemmas.
\jm{fix this:} The first lemma shows that if we execute any instruction next
from any concrete state, the invariant is preserved between the
new concrete state and an abstract state based on the
borrow checker rules.
This state must be in the $\below$ relation with
with the next program annotation.
We next use another lemma relating $\below$ and
the invariant to prove the theorem.

\begin{manuallemma}{1}
\label{type-weakening-lemma}
Let $\concState =  (P,M)$ be a concrete state with non-empty call stack
$P = \st{\proc,\pc, L_1,  S_1}\cons P_0$.
Let 
$\absState =  \abs{\concState} =  \st{\proc,\pc, \hat{L}_1,  \hat{S}_1,B_1}\cons \abs{P_0}$
be the corresponding abstract state.   If
\begin{itemize}
\item
$\inv(\concState,  \absState)$
\item
$\st{\hat{L}_1,\hat{S}_1,B_1} \below \st{\hat{L}_2,\hat{S}_2,B_2}$
\end{itemize}
then
$\inv(\concState, \st{\proc,\pc, \hat{L}_2,  \hat{S}_2,B_2}\cons \abs{P_0})$.
\end{manuallemma}
\jm{Is it necessary that $\absState =  \abs{\concState}$ or is \\
$\inv(\concState,  \st{\proc,\pc, \hat{L}_1,  \hat{S}_1,B_1}\cons \abs{P_0})$ sufficient?}

\begin{proof}[Proof of Lemma \ref{type-weakening-lemma}]
If  $\st{\hat{L}_1,\hat{S}_1,B_1} \below \st{\hat{L}_2,\hat{S}_2,B_2}$
then by definition of $\below$ it follwos that $\hat{L}_1 = \hat{L}_2$,  $\hat{S}_1 = \hat{S}_2$,
and each edge in $B_1$ is subsumed by some edge in $B_2$.
Thus, the call stacks and operand stacks of $\absState_1$ and $\absState_2$ are identical
and each edge in the global borrow graph of $\absState_1$ is subsumed by some edge in
the global  borrow graph of $\absState_2$.
The preservation of $\inv$ follows from the definition of subsumption of
a borrow edge.
\end{proof}



\begin{manuallemma}{2}
\label{type-sound-lemma-local}
Let $\concState =  (P,M)$ be a concrete state with call stack
$P = \st{\proc,\pc, L_1,  S_1}\cons P_0$.
Let 
$\absState =  \abs{\concState} =  \st{\proc,\pc, \hat{L}_1,  \hat{S}_1,B_1}\cons \abs{P_0}$
be the corresponding abstract state.   If
\begin{itemize}
\item
$\inv(\concState,  \absState)$
\item
$\program \vdash \concState \rightarrow \concState'$ by a local instruction
\item
$\proc,\bcodes{\proc}[\pc] \vdash \lstates{\proc}[\pc] \rightarrow
\st{\hat{L},\hat{S},B}$
\end{itemize}
then
$\inv(\concState, \st{\proc,\pc, \hat{L}_2,  \hat{S}_2,B_2}\cons \abs{P_0})$.
\end{manuallemma}


\begin{manuallemma}{3}
\label{type-sound-lemma}
Let $\concState$ be a concrete state with corresponding abstract state
$\absState =  \abs{\concState}$.
If
\begin{itemize}
\item
$\inv(\concState,\abs{\concState})$
\item
$\program \vdash \concState \rightarrow \concState'$
\end{itemize}
with 
$\concState' =  (P',M')$ and 
$P' = \st{\proc',\pc', L',  S'}\cons P'_0$.
Then there exists $\st{\hat{L},\hat{S},B}$
such that
\begin{itemize}
\item
$\inv(s', \st{\hat{L},\hat{S},B}\cons \abs{P'_0})$
\item
$\st{\hat{L},\hat{S},B} \below \lstates{\proc'}[\pc']$.
\end{itemize}
\end{manuallemma}

\begin{proof}[Proof of Lemma \ref{type-sound-lemma}]
If $\program \vdash \concState \halfstep \concState'$ by a local instruction,
then $\Base(\concState) = \Base(\concState')$ and
we get the result from Lemma~\ref{type-sound-lemma-local}
and the definition of $\program$ being well-typed.
The case for $\branchCmd$ is similar.

Suppose $\program \vdash \concState \halfstep \concState'$ via
$\ao{\callCmd}{\proc'}$.
We argue
$\inv(\concState',\Base(\concState') \dagger \lstates{\proc'}[0])$ holds.
The proof follows since $\below$ is reflexive.

Suppose $\program \vdash \concState \halfstep \concState'$ via
$\returnCmd$ and $\bcodes{\proc}[\pc] = \ao{\callCmd}{\proc'}$.
Suppose
$\abs{\concState'} = \Base(\concState') \dagger \st{\hat{L}_1,\hat{S}_1,B_1}$.
Then, we know that
$\bcodes{\proc}[\pc - 1] = \ao{\callCmd}{\proc'}$,
$\lstates{\proc}[\pc - 1] = \st{\hat{L}_1,\hat{S}_1,B_1}$, and
there exists $\st{\hat{L}_2,\hat{S}_2,B_2}$ such that
$\proc, \ao{\callCmd}{\proc'} \vdash \st{\hat{L}_1,\hat{S}_1,B_1} \rightarrow \st{\hat{L}_2,\hat{S}_2,B_2}$.
We argue that $\inv(\concState',\Base(\concState') \dagger \st{\hat{L}_2,\hat{S}_2,B_2})$
holds using the typing argument
for $\returnCmd$ in $\proc'$ and $\ao{\callCmd}{\proc'}$ in $\proc$.
Since $\program$ is well-typed, we also know that $\st{\hat{L}_2,\hat{S}_2,B_2} \subseteq \lstates{\proc}[\pc]$
and the proof follows.
\end{proof}

Lemmas~\ref{type-sound-lemma-local} and~\ref{type-sound-lemma}
are combined to prove the Theorem~\ref{type-sound-thm}.
\begin{manualtheorem}{1}
\label{type-sound-thm}
Let program $\program$ be well-typed.
If $\concState$ is a concrete state with $\inv(\concState,\abs{\concState})$
and $\program \vdash \concState \rightarrow \concState'$,
then $\inv(\concState',\abs{\concState'})$.
\end{manualtheorem}

\begin{proof}[Proof of Theorem \ref{type-sound-thm}]
Let program $\program$ be well-typed.
Let $\concState$ be a concrete state with $\inv(\concState,\abs{\concState})$
and $\program \vdash \concState \rightarrow \concState'$.
If the transition is due to \rulename{Emp}, the call stack
and operand stack in $\concState'$ are both empty.
Therefore, $\abs{\concState'} = \st{[],[],\{\}}$ and
$\inv(\concState',\abs{\concState'})$ holds trivially.

In all cases other than \rulename{Emp}, the call stack in $\concState'$
is nonempty.
Let $\concState \halfstep \concState^-$ and let the top frame of
the call stack of $\concState'$ be $\st{\proc,\pc,\_}$.
We use Lemma~\ref{type-sound-lemma} to find
$\st{\hat{L},\hat{S},B} \below \lstates{\proc}[\pc]$
such that $\inv(\concState^-,\Base(\concState^-) \dagger \st{\hat{L},\hat{S},B})$.
We use Lemma~\ref{type-weakening-lemma} to conclude that
$\inv(\concState^-,\Base(\concState^-) \dagger \lstates{\proc}[\pc])$.
By replacing the program counter in the top frame of the call stack of
$\concState^-$, we get $\concState'$.
By replacing the program counter in the top frame of the call stack of
$\Base(\concState^-) \dagger \lstates{\proc}[\pc])$,
we get $\abs{\concState'}$.
Therefore, we get $\inv(\concState', \abs{\concState'})$.
\end{proof}

\begin{proof}[Proof of Lemma \ref{type-sound-lemma-local}]
Let
$\absState  = \abs{\concState}  = \st{\stackht{(\proc, \pc, \hat{L})}{\hat{P}},\hat{S},B}$.
Note that $\absState$ has the same procedure name and program counter
in the top of the call stack as $\concState$.
We note that
$\absState = \Base(\concState) \dagger \lstates{\proc}[\pc]$.
Let $\lstates{\proc}[\pc] = \st{\hat{L}_0,\hat{S}_0,B_0}$.
Let $\absState' = \Base(\concState) \dagger \st{\hat{L},\hat{S},B}$.
We must show $\inv(\concState',\absState')$.
The proof proceeds by case analysis according to the
local instruction that is executed to reach $\concState'$.
There are four parts of the invariant to check for each instruction:
type agreement, no memory leaks, no dangling references, and referential transparency.
The first two conditions are straightforward for all local instructions and are
therefore omitted from this presentation of the proof.

\paragraph{$\ao{\borrowlocCmd}{x}$.}
Suppose $\bcodes{\proc}(\pc) = {\ao{\borrowlocCmd}{x}}$ with $\lread{L}{x}=c$.
This instruction pushes a reference to $c$ on top of the operand stack.
The operational semantics give us
\[
\concState' = \st{\stackht{(\proc, \pc, L)}{P},\stackht{\rft{c}{[]}}{S},M}.
\]
The rule for $\ao{\borrowlocCmd}{x}$ shows
$\lread{\hat{L}_0}{x} = t$ for $t \in \valtype$,
$\hat{L} = \hat{L}_0$,
$\hat{S} = \stackht{\mut{t}}{\hat{S}_0}$, and
$B = \factor{B_0}{\psloc(0,x)}{\osloc(\len{\hat{S}_0})}$.
Thus, $B$ is derived from $B_0$ by
\begin{enumerate}
\item adding the edge $Borrow(\psloc(0,x),{\varepsilon},{\osloc(\len{\hat{S}_0})})$, and
\item replacing each edge $Borrow(\psloc(0,x),p,n)$ by the edge
$Borrow(\osloc(\len{\hat{S}_0}),p,n)$.
\end{enumerate}

\noindent {\em No dangling references.}
The only new position in $\abs{\concState'}$ is the new top of the operand stack
containing a mutable reference.
The new borrow edge $Borrow(\psloc(0,x),{\varepsilon},{\osloc(\len{\hat{S}})}$
incident on this position is realized.
Also, any realized borrow edge leaving $\psloc(0,x)$ that was moved to leave from
$\osloc(\len{\hat{S}})$ continues to be a realized edge.
Therefore the property holds for $\concState'$ and $\absState'$.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the new location $\osloc(\len{\hat{S}})$.

Let $m \neq \osloc(\len{\hat{S}})$ and $n \neq \osloc(\len{\hat{S}})$.
This case works because the factor operation is such that any realizable path
that went through $\psloc(0,x)$
now goes through both $\psloc(0,x)$ and $\osloc(\len{\hat{S}})$.

If $m=\osloc(\len{\hat{S}})$,
then $\concState(\psloc(0,x)) < \concState(n)$.
There is a realizable path in $\concState$ from $\psloc(0,x)$ to $n$ by induction.
This path can be transformed into a realizable path in $\concState'$
that goes through $\osloc(\len{\hat{S}})$.

If $n=\osloc(\len{\hat{S}})$,
then either $m = \psloc(0,x)$ or $\concState(m) = \concState'(m) = \concState'(n)$.
In the first case, the required path is simply the new $\varepsilon$-edge.
In the second case,
there is a realizable path in $\concState$ from $\psloc(0,x)$ to $m$ by induction.
This path can be transformed into a realizable path in $\concState'$
that goes through $\osloc(\len{\hat{S}})$.

\paragraph{$\ao{\borrowfieldCmd}{f,x}$.}
Suppose $\bcodes{\proc}(\pc) = \ao{\borrowfieldCmd}{f,x}$ with $\lread{L}{x} = \rft{c}{p}$.
There are two cases, based on whether $\lread{\hat{L}_0}{x} = \mut{\record{(f,t),\ldots}}$ or
$\lread{\hat{L}_0}{x} = \imm{\record{(f,t),\ldots}}$.
In both cases,
the instruction pushes a reference $\rft{c}{p::f}$ derived from
$\lread{L}{x}$ on top of the operand stack.
The operational semantics gives us
 \[
\concState' = \st{\stackht{(\proc, \pc, L)}{P},\;\stackht{\rft{c}{p::f}}{S},\;M}.
\]
However, the static analysis differs in the two cases.
We prove each case separately.

\noindent {\em Case 1.}
Suppose $\lread{\hat{L}_0}{x} = \mut{\record{(f,t),\ldots}}$ is a mutable reference.
The corresponding borrow-checker rule shows
$\hat{L} = \hat{L}_0$,
$\hat{S}= \stackht{\mut{t}}{\hat{S}_0}$, and
$B = \factorf{f}{B_0}{\psloc(0,x)}{\osloc(\len{\hat{S}})}$.
This borrow graph operation \emph{fails} and the bytecode program is rejected
if there is any edge labeled $\varepsilon$ or $*$
coming out of $\psloc(0,x)$ in $B_0$.
We therefore assume there is no such edge in $B_0$ and
derive $B$ from $B_0$ by
\begin{itemize}
\item Adding the edge $Borrow(\psloc(0,x),{f},{\osloc(\len{\hat{S}})}$, and
\item Replacing each edge $Borrow(\psloc(0,x),\concat{f}{p},n)$ by the edge $Borrow(\osloc(\len{\hat{S}},p,n)$.
\end{itemize}

\noindent {\em No dangling references.}
This proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the new location $\osloc(\len{\hat{S}})$.

If $m \neq \osloc(\len{\hat{S}})$ and $n \neq \osloc(\len{\hat{S}})$,
then the proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

If $m=\osloc(\len{\hat{S}})$, then $\concState(\psloc(0,x)) < \concState(n)$.
There is a realizable path in $\concState$ from $\psloc(0,x)$ to $n$ by induction.
Since there is no edge labeled $\varepsilon$ or $*$ out of $\psloc(0,x)$,
this path must follow one of the factored edges.
Therefore, this path can be transformed to go through $\osloc(\len{\hat{S}})$
in $\concState'$.

If $n=\osloc(\len{\hat{S}})$,
then $\concState(m) < \concState(\psloc(0,x))$
or $\concState(\psloc(0,x)) = \concState(m)$
or $\concState(\psloc(0,x)) < \concState(m)$.
In the first case,
there is a realizable path in $\concState$ from $m$ to $\psloc(0,x)$ by induction.
We can extend this path to $n$ by using the realizable edge from $\psloc(0,x)$ to
$\osloc(\len{\hat{S}})$.
In the second case,
there must be a realizable path either from $m$ to $\psloc(0,x)$ or from
$\psloc(0,x)$ to $m$ by induction.
Since there is no edge labeled $\varepsilon$ or $*$ out of $\psloc(0,x)$,
the realizable path must be from $m$ to $\psloc(0,x)$.
We can extend this path to $n$ by using the realizable edge from $\psloc(0,x)$ to
$\osloc(\len{\hat{S}})$.
In the third case, $\concState(m) = \concState'(m) = \concState'(n)$ and
there is a realizable path in $\concState$ from $\psloc(0,x)$
to $m$ by induction.
Since there is no edge labeled $\varepsilon$ or $*$ out of $\psloc(0,x)$,
this path must follow one of the factored edges.
Therefore, this path can be transformed to go through $\osloc(\len{\hat{S}})$
in $\concState'$.

\noindent {\em Case 2.}
Suppose $\lread{\hat{L}_0}{x} = \imm{\record{(f,t),\ldots}}$ is an immutable reference.
The corresponding borrow-checker rule shows
$\hat{L} = \hat{L}_0$,
$\hat{S}= \stackht{\imm{t}}{\hat{S}_0}$, and
$B = B_0 \cup \{\Borrow(\psloc(0,x),f,\osloc(\len{\hat{S}})\}$.

\noindent {\em No dangling references.}
This proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the new location $\osloc(\len{\hat{S}})$.

If $m \neq \osloc(\len{\hat{S}})$ and $n \neq \osloc(\len{\hat{S}})$,
then the proof works exactly like the corresponding proof for $\ao{\borrowlocCmd}{x}$.

If $m=\osloc(\len{\hat{S}})$,
then $\concState(\psloc(0,x)) < \concState(n)$.
We get $\concState(n) \in \immreftype$ by induction.

If $n=\osloc(\len{\hat{S}})$,
then $\concState(m) < \concState(\psloc(0,x))$
or $\concState(m) = \concState(\psloc(0,x))$
or $\concState(\psloc(0,x)) < \concState(m)$.
In the first case, by induction (instantiating $m$ with $m$ and $n$ with $\psloc(0,x)$),
either $\concState(m) \in \immreftype$ or
$\concState(m) \not \in \immreftype$ and there is a realizable path in $\concState$ from
$m$ to $\psloc(0,x)$ which can be extended to a realizable path in $\concState'$ to $n$.
In the second case, by induction (instantiating $m$ with $\psloc(0,x)$ and $n$ with $m$),
either $\concState(m) \in \immreftype$ or
$\concState(m) \not \in \immreftype$ and there is a realizable path in $\concState$ from
$m$ to $\psloc(0,x)$ which can be extended to a realizable path in $\concState'$ to $n$.
In the third case, we get $\concState(m) \in \immreftype$ by induction.

\paragraph{$\ao{\movelocCmd}{x}$.}
Vertices in the borrow graph
are renamed from the old position of the moved value to its new position.
The new position does not appear as the source or target of any borrow
edge in the borrow graph.
Therefore, the new borrow graph is isomorphic to the old borrow graph.
Properties (No dangling references) and  Referential transparency) follow
from the fact that these properties held before this instruction was executed.

\paragraph{$\popCmd$.}
The analysis pops the top of the abstract operand stack and
eliminates the location corresponding to it using the
$\mathit{elim}$ operation on borrow graphs.
This operation eliminates location $u$ in $B_0$ as follows:
(1)~For every edge $\Borrow(a,p,u)$ coming into $u$ and edge $\Borrow(u,q,b)$
going out of $u$, add an edge $\Borrow(a,\concat{p}{q},b)$.
(2)~Delete all edges coming into and going out of $u$.
This ensures that all transitive borrow relationships
going through the reference that has been popped off the operand stack are
maintained,
preserving (No dangling references) and (Referential transparency) as a result.

\paragraph{$\ao{\storelocCmd}{x}$.}
The proof is a combination of the
proof for $\ao{\movelocCmd}{x}$ and $\popCmd$.

\paragraph{$\ao{\copylocCmd}{x}$.}
The proof is similar to $\ao{\borrowlocCmd}{x}$
in case the variable $x$ being copied is a reference.
Otherwise,
there is no change in the borrow graph and the proof is straightforward.

\paragraph{$\writerefCmd$.}
The proof is similar to $\popCmd$.

\paragraph{$\freezerefCmd$.}
The operational semantics gives us $\concState' = \concState$.
If the reference on top of the abstract operand stack in $\abs{\concState}$
is immutable, the local abstract state does not change and the proof is done.
Otherwise, the freezable mutable reference at the top of the abstract operand
stack is converted into an immutable reference.

\noindent {\em No dangling references.}
This proof is straightforward since there is no change in the borrow graph.

\noindent {\em Referential transparency.}
We need to check all $m,n\in\dom{\absState'}$ such that
$\absState'(n) \in \reftype$ and $\concState'(m) \leq \concState'(n)$.
There are three cases depending on whether one of $m$ or $n$
is the location $\osloc(\len{\hat{S}}-1)$.

If $m \neq \osloc(\len{\hat{S}}-1)$ and $n \neq \osloc(\len{\hat{S}}-1)$,
then the proof is straightforward.

Suppose $m=\osloc(\len{\hat{S}}-1)$.
By induction, either
(1)~there is a path realizable in $\concState$ from $m$ to $n$, or
(2)$\concState(m) = \concState(n)$ and there is a path realizable
in $\concState$ from $n$ to $m$.
In the first case, the freezability of $m$ and Lemma~\ref{no-path-imm-to-mut}
indicate that $\absState(n) \in \immreftype$.
Since $\absState(n) = \absState'(n)$, we are done.
In the second case, we can reuse the path since $\concState = \concState'$.

Suppose $n=\osloc(\len{\hat{S}}-1)$.
By induction, either
(1)~$\absState(m) \not \in \immreftype$ and there is a path realizable
in $\concState$ from $m$ to $n$, or
(2)$\concState(m) = \concState(n)$ and there is a path realizable
in $\concState$ from $n$ to $m$.
In the first case, we can reuse the path since $\concState = \concState'$ and
$\absState(m) = \absState'(m)$.
In the second case, the freezability of $n$ and Lemma~\ref{no-path-imm-to-mut}
indicate that $\absState(m) \in \immreftype$.
Since $\absState(m) = \absState'(m)$, we are done.

\paragraph{$\readrefCmd$.}
The proof is similar to $\popCmd$.

We omit discussion of $\packCmd$, $\unpackCmd$, and $\stackopCmd$
since these instructions do not perform any reference-related operations.
\end{proof}

\subsection*{Old version, for comparison}
To aid our proof, we define an auxiliary transition relation
$\program \vdash \concState \halfstep \concState$.
We view a transition $\program \vdash \concState \rightarrow \concState'$
as happening in two steps.
In the first step, the instruction pointed to by the program counter at
the top of the call stack in $\concState$ is executed to change parts
of the state to yield $\concState^-$
without adjusting the program counter to point to the next instruction.
In the second step, the program counter in $\concState^-$
is adjusted to yield $\concState'$ and move to the next instruction.
We write $\program \vdash \concState \halfstep \concState^-$
to denote the first part of this two-step process.
The concrete states $\concState^-$ and $\concState'$
coincide in the two cases when
the call stack in $\concState'$ is empty or
$\concState'$ is obtained from $\concState$ by executing a
call instruction;
in these two cases,
$\program \vdash \concState \rightarrow \concState'$
is a single step.

The following two lemmas together state that the transformation
of the abstract state when a local instruction is executed preserves $\inv$.
The proof of Lemma~\ref{type-sound-lemma-local}
is provided later in this document.
\begin{manuallemma}{2-old}
%\label{type-sound-lemma-local}
If
\begin{itemize}
\item
$\concState = \st{\stackht{(\proc, \pc, \_)}{\_},\_,\_}$
\item
$\inv(\concState,\abs{\concState})$
\item
$\program \vdash \concState \halfstep \concState'$ by a local instruction
\item
$\proc,\bcodes{\proc}[\pc] \vdash \lstates{\proc}[\pc] \rightarrow
\st{\hat{L},\hat{S},B}$
\end{itemize}
then
$\inv(\concState',\Base(\concState) \dagger \st{\hat{L},\hat{S},B})$.
\end{manuallemma}

\begin{manuallemma}{3-old}
%\label{type-sound-lemma}
If
\begin{itemize}
\item
$\inv(\concState,\abs{\concState})$
\item
$\program \vdash \concState \halfstep \concState'$
\item
$\program \vdash \concState \rightarrow (\stackht{\st{\proc,\pc,\_}}{\_},\_,\_)$
\end{itemize}
then there exists $\st{\hat{L},\hat{S},B}$
such that
\begin{itemize}
\item
$\inv(s',\Base(s') \dagger \st{\hat{L},\hat{S},B})$
\item
$\st{\hat{L},\hat{S},B} \below \lstates{\proc}[\pc]$.
\end{itemize}
\end{manuallemma}
